A Survey on Signed Graph Embedding: Methods and Applications

A signed graph (SG) is a graph where edges carry sign information attached to it. The sign of a network can be positive, negative, or neutral. A signed network is ubiquitous in a real-world network like social networks, citation networks, and various technical networks. There are many network embedding models have been proposed and developed for signed networks for both homogeneous and heterogeneous types. SG embedding learns low-dimensional vector representations for nodes of a network, which helps to do many network analysis tasks such as link prediction, node classification, and community detection. In this survey, we perform a comprehensive study of SG embedding methods and applications. We introduce here the basic theories and methods of SGs and survey the current state of the art of signed graph embedding methods. In addition, we explore the applications of different types of SG embedding methods in real-world scenarios. As an application, we have explored the citation network to analyze authorship networks. We also provide source code and datasets to give future direction. Lastly, we explore the challenges of SG embedding and forecast various future research directions in this field.

==> network_analysis.tex <==
\section{\LARGE Benchmark Datasets and Source Code}
In previous works, most of the research on signed networks applied their proposed models on four real world directed signed network dataset:
\begin{itemize}
\item{Bitcoin-Appha \cite{kumar2016structure}:This is who-trusts-whom network of people who trade using Bitcoin on a platform called Bitcoin Alpha.}
\item{Bitcoin-OTC \cite{kumar2016structure}:This is who-trusts-whom network of people who trade using Bitcoin on a platform called Bitcoin OTC.}
\item{Slashdot \cite{leskovec2010signed}:Slashdot is a technology-related news website know for its specific user community. The website features user-submitted and editor-evaluated current primarily technology oriented news. }
\item{Epinions \cite{leskovec2010signed}:This is who-trust-whom online social network of a a general consumer review site Epinions.com.}

\end{itemize}

\begin{table*}[h!] \setlength\tabcolsep{0.1pt} 
% \captionsetup{justification=right}
\caption{A summary of commonly used signed graph datasets}
\centering
\scalebox{0.85}{
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 
\renewcommand{\arraystretch}{2}
% \caption{Sample Table.}\label{tab1} 

\begin{tabular}{|p{2.7cm}|p{2.5cm}|p{2.5cm}|p{3cm}|p{2.5cm}|p{6cm}|}
\hline
% \multicolumn{1}{|p{2.7cm}|}{Dataset} & 
% \multicolumn{1}{p{2.5cm}|}{\centering Link Prediction} & 
% \multicolumn{1}{p{2.5cm}|}{\centering Node Clustering} & 
% \multicolumn{1}{p{2.5cm}|}{\centering Community Detection & 
% \multicolumn{1}{p{2.5cm}|}{\centering Node Classification} & 
% \multicolumn{1}{p{6cm}|}{\centering Related Papers} \\
% \begin{tabular}{|p{2.7cm}|{\centering p{2.5cm}}|{\centering p{2.5cm}}|{\centering p{2.5cm}}|{\centering p{2.5cm}}|p{6cm}|}
% {|l|l|l|l|l|l|} 
% \hline

\textbf{Dataset} & \textbf{Link Prediction} & \textbf{Node Clustering} & \textbf{Community Detection} & \textbf{Node Classification} & \textbf{Related Papers} \\
 \hline\hline
 
Bitcoin-Alpha \cite{kumar2016structure} & $\checkmark$ & $\checkmark$ &   &  &\cite{li2020learning,mara2020csne,grover2016node2vec,rahaman2018method,derr2018signed} \\ \hline
Bitcoin-OTC \cite{kumar2016structure} & $\checkmark$ &  & $\checkmark$ &   &\cite{li2020learning,mara2020csne,derr2018signed,rahaman2018method} \\ \hline
Slashdot \cite{leskovec2010signed} & $\checkmark$ &  &  & $\checkmark$&  \cite{dhelim2020compath,wang2017attributed,li2020learning,kim2018side,wang2017signed,yuan2017sne,mara2020csne,song2018learning,grover2016node2vec,rahaman2018method,kim2018side,derr2018signed}  \\ \hline
Epinions \cite{leskovec2010signed} & $\checkmark$  & $\checkmark$  & $\checkmark$ & $\checkmark$   &\cite{wang2017attributed},\cite{dhelim2020compath,li2020learning,kim2018side,wang2017signed,kim2018side,mara2020csne,grover2016node2vec,song2018learning,rahaman2018method,derr2018signed} \\ \hline
Wiki \cite{leskovec2010signed} & $\checkmark$  &  &  &$\checkmark$  &\cite{kim2018side,yuan2017sne,mara2020csne,song2018learning,wang2018shine,rahaman2018method} \\ \hline
Newsfullness \cite{leskovec2010signed} &  &  & $\checkmark$ &  &\cite{dhelim2020compath} \\ \hline
\end{tabular}}
\end{table*}
\indent
In our work, we are using citation network for different kind of research domains. Currently, we have explored Data Mining conferences and Software Engineering conferences. The dataset have been extracted from Google Scholar from timeline 2012 to 2022. We have collected 3000 research articles from each domain.  We have created authorship network from the dataset and currently building the citation network based on the papers have been cited in the 3000 research articles. 

\begin{table*}[h!] \setlength\tabcolsep{0.1pt} 
% \captionsetup{justification=right}
\caption{Source code of related models}
\centering
\scalebox{0.75}{
% \def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 
\renewcommand{\arraystretch}{2}
% \caption{Sample Table.}\label{tab1} 

\begin{tabular}{|p{2.5cm}|p{15cm}|p{2.5cm}|}
\hline

\textbf{Paper} & \textbf{Source Code} & \textbf{Programming Platform} \\
 \hline\hline
 SGCN\cite{derr2018signed} & \url{https://github.com/benedekrozemberczki/SGCN}  & PyTorch \\
 \hline
% SiNE\cite{wang2017signed} & Structural Balance Theory & Embedding \\
\hline
% SNE\cite{yuan2017sne} & Similarity Measure & Embedding \\ 
\hline
SIGNet\cite{islam2018signet} & \url{https://github.com/raihan2108/signet} & Python and C++ \\
 \hline
% SNEA\cite{wang2017attributed} & Extended Structural Balance Theory  & Embedding \\
 \hline
SiHet\cite{rizi2020signed} & \url{https://github. com/fatemehsrz/SiHet} & Python\\
\hline
DNE-SBP \cite{shen2018deep} & \href{https://github.com/shenxiaocam/Deep-network-embedding-for-graph-representation-learning-in-signed-networks}{DNE-SBP} & MATLAB \\
\hline
SIDE\cite{kim2018side} &  \url{https://datalab.snu.ac.kr/side/} & Python \\
\hline
% SHINE \cite{wang2018shine} & Structural balance theory & Embedding \\
% \hline
% ComPath \cite{dhelim2020compath} & Proximity between vertex & Embedding \\
% \hline
% SGNS \cite{wang2018shine} & Structural balance theory and similarity measure & Embedding \\
% \hline
% SNEGAN \cite{wang2018shine} & Structural balance theory and similarity measure &  Embedding \\
% \hline
StEM \cite{rahaman2018method} & \url{https://github.com/InzamamRahaman/StEMPublic} &  Python \\
\hline
nSNE \cite{song2018learning} & \url{https://github.com/wzsong17/Signed-Network-Embedding} &  PyTorch \\
\hline
% CSNE \cite{mara2020csne} & Structural balance &  Embedding \\
% \hline
SiGAT \cite{huang2019signed} & \url{https://github.com/huangjunjie95/SiGAT} &  Python \\
\hline
\end{tabular}}
\end{table*}

% \begin{table*}[h!] \setlength \tabcolsep{0.1pt} % you can change 0.1pt to maximum 9 pt, as you asked for IEEE
% \caption{A summary of commonly used signed graph datasets}
% % \begin{center}
% % \scalebox{0.85}

% \def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 
% \renewcommand{\arraystretch}{2}
% \resizebox{17cm}{!}{

% \begin{tabularx}{1\textwidth}{|p{2.5cm}|{\centering p{4cm}}|{\centering p{4cm}}|{\centering p{4cm}}|{\centering p{4cm}}|{p{4cm}}}
% \hline
% \textsc{\textbf{Dataset}} & \textsc{\textbf{Link Prediction}} & \textsc{\textbf{Node Clustering}} &  \textsc{\textbf{Community Detection}} & \textsc{\textbf{Node Classification}}  & \textsc{\textbf{Related Papers}}\\ \hline
% Bitcoin-Alpha \cite{kumar2016structure} & $\checkmark$ & $\checkmark$ &  &  &\cite{li2020learning,mara2020csne,grover2016node2vec,rahaman2018method,derr2018signed} \\ \hline
% Bitcoin-OTC \cite{kumar2016structure} & $\checkmark$ &  & $\checkmark$ &   &\cite{li2020learning,mara2020csne,derr2018signed,rahaman2018method} \\ \hline
% Slashdot \cite{leskovec2010signed} & $\checkmark$ &  &  & $\checkmark$&  \cite{dhelim2020compath,wang2017attributed,li2020learning,kim2018side,wang2017signed,yuan2017sne,mara2020csne,song2018learning,grover2016node2vec,rahaman2018method,kim2018side,derr2018signed}  \\ \hline
% Epinions \cite{leskovec2010signed} & $\checkmark$  & $\checkmark$  & $\checkmark$ & $\checkmark$   &\cite{wang2017attributed},\cite{dhelim2020compath,li2020learning,kim2018side,wang2017signed,kim2018side,mara2020csne,grover2016node2vec,song2018learning,rahaman2018method,derr2018signed} \\ \hline
% Wiki \cite{leskovec2010signed} & $\checkmark$  &  &  &$\checkmark$  &\cite{kim2018side,yuan2017sne,mara2020csne,song2018learning,wang2018shine,rahaman2018method,kim2018side} \\ \hline
% Newsfullness \cite{leskovec2010signed} &  &  & $\checkmark$ &  &\cite{dhelim2020compath} \\ \hline
% \hline
% \end{tabularx}}
% % \end{center}
% \end{table*}




\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{images/Picture1.png}
    % \caption{Authorship Network}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth,height=4.93cm]{images/Picture2.png}
    % \caption{Author Profile}
  \end{minipage}
  \caption{\footnotesize \raggedright The left image depicts authorship network within same domain and the right image depicts the author profile information}
\end{figure}
\begin{figure}
\centering
    \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/wordcloud_title_data_mining.jpeg}
    \caption{\footnotesize Wordcloud of Data Mining}
    \end{subfigure}
\hspace{5mm}
    \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/wordcloud_title_soft_engg.jpeg}
    \caption{\footnotesize Wordcloud of Software Engineering}
    \end{subfigure}
\end{figure}


% \begin{figure}
% \centering
%     \begin{subfigure}
%     \includegraphics[width=8cm]{images/wordcloud_title_data_mining.jpeg}
%     \caption{\footnotesize Wordcloud of Data Mining}
%     \end{subfigure}
% \vspace*{3mm}
%     \begin{subfigure}
%     \includegraphics[width=8cm]{images/wordcloud_title_soft_engg.jpeg}
%     \caption{\footnotesize Wordcloud of Software Engineering}
%     % \caption{The top and bottom image shows the most frequent words used in the articles title in data mining conferences and software engineering conferences correspondingly.}
%     \end{subfigure}
% \end{figure}



\section{\LARGE Network Analysis}

For the purpose of generating explanations of networks, we have considered a diverse set of features. These features gives a broader knowledge of the network and also might give some important aspects which can be useful for our future works. 

In this section, we have tried to answer below research questions:
\begin{itemize}
  \item How authors are connected within domain from different conferences?
  \item  How is the pattern of paper published for different research domain?
  \item How network feature are distinct for research domains?
  \item Can we find the most influential authors within a domain?
  \item Can we identify the most frequently affiliated organization within a domain?
\end{itemize}

\begin{table}[!h]
% {\renewcommand \arraystretch{0.05}
\caption{Network Features}
\begin{tabular}{|l|c|c|l|l||} \hline
Features & Data Mining & Software Engg  \\ \hline\hline
No of nodes &3538 & 2499  \\ \hline
No of edges &4397 &  2978  \\ \hline
Strongly cc& 3325 & 2394 \\ \hline
Weakly cc& 893 & 586 \\ \hline
Largest cc nodes & 982 & 729 \\ \hline
Largest strongly cc nodes & 172 & 12 \\ \hline
Percentage of strongly cc & 3.72\% & 0.48\% \\ \hline
\end{tabular}
\end{table}

\subsection{Definitions}
\begin{itemize}
  \item Connected Component: A connected component or simply component of an undirected graph is a subgraph in which each pair of nodes is connected with each other via a path.
  \item Strongly Connected Component:  A strongly connected component is the portion of a directed graph in which there is a path from each vertex to another vertex. It is applicable only on a directed graph.
  \item Weakly Connected Component: Given a directed graph, a weakly connected component (WCC) is a subgraph of the original graph where all vertices are connected to each other by some path, ignoring the direction of edges.
\end{itemize}
From the table 4, we can see the largest connected component is relatively larger in data mining conference, which means the authors are connected and co-authored together a lot more than the software engineering conferences authors.

% \begin{figure}
% \centering
%     \begin{subfigure}
%     \includegraphics[width=9cm]{images/largest_DM.png}
%     \caption{\footnotesize Network of 982 author nodes in Data Mining}
% \end{subfigure}
% \vspace*{3mm}
% \begin{subfigure}
%     \includegraphics[width=9cm]{images/largest_sw.png}
%     \caption{\footnotesize Network of 729 author nodes in Software Engineering}
%     % \caption{The top and bottom image shows the most frequent words used in the articles title in data mining conferences and software engineering conferences correspondingly.}
% \end{subfigure}
% \end{figure}


\begin{figure}[!tbp]
\centering
  \begin{minipage}[b]{.5\textwidth}

    \includegraphics[width=\textwidth]{images/largest_DM.png}
    \caption{Network of 982 author nodes in Data Mining}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.53\textwidth}
    \includegraphics[width=\textwidth]{images/largest_sw.png}
    \caption{Network of 729 author nodes in Software Engineering}
  \end{minipage}
  \caption{The left image depicts authorship network within same domain and the right image depicts the author profile information}
\end{figure}

For each citation network, the citation pattern reveals how the citation culture developed within the domain. The pattern gives insights into data mining citation patterns. 

From the degree rank plot analysis (Figure 16, 17), we can see that authors in the largest connected component have the highest degree of value of 40 and rank 1000 in data mining conferences, whereas software engineering conferences authors have the highest degree value of 20 and rank 700. From degree histogram of the network, we can see that more than 200 author nodes have an average degree value of 5 in data mining, and in software engineering, more than 200 author nodes have an average degree of 2.5. 


% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{.4\textwidth}
%     \includegraphics[width=\textwidth]{images/data_mining_citation_pattern.png}
%     % \caption{Authorship Network}
%   \end{minipage}
% %   \hfill
%   \begin{minipage}[b]{.4\textwidth}
%     \includegraphics[width=\textwidth]{images/software_engineering_citation_pattern.png}
%     % \caption{Author Profile}
%   \end{minipage}
%   \caption{The top image depicts publication trend network in Data Mining domain and the bottom image depicts publication trend in Software Engineering domain}
% \end{figure}

The authors in the conferences have worked as coauthored multiple times. We have captured the strongest connected coauthors who have worked together more frequently from both domains (Figure 18).

\begin{figure}[!tbh]
  \centering
  \begin{minipage}[b]{0.50\textwidth}
\includegraphics[width=\textwidth,height=10cm]{images/dm_strongcc.png}
    \centering(a)
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.50\textwidth}
    \includegraphics[width=\textwidth,height=8cm]{images/se_strongcc.png}
    \centering{(b)}
  \end{minipage}
  \caption{\footnotesize The most influential authors (a) Data Mining (b) Software Engineering }
\end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.32\textwidth}
%     \includegraphics[width=\textwidth]{images/dm_strongcc.png}
%     % \caption{Authorship Network}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\textwidth}
%     \includegraphics[width=\textwidth,height=4.93cm]{images/se_strongcc.png}
%     % \caption{Author Profile}
%   \end{minipage}
%   \caption{The top and bottom image show the strongly connected authors coauthored together in data mining and software engineering correspondingly. }
% \end{figure}

Also, authors publish papers at the same conferences every year. From the number of total papers published within the research domain, we are able to mark the most influential authors within the domain. We have come up with the most 10 influential authors from both domains. The top most influential authors in data mining are Huan Liu, Jiawei Han, Philip S. Yu so, and so forth. Similarly, the top most influential authors in software engineering are David Lo, Mark Harman, Barbara Ann Kitchenham, Claes Wohlin, Nachiappan Nagappan so, and so forth (Figure 21). 

\begin{figure}[!tbh]
  \centering
  \begin{minipage}[b]{0.36\textwidth}
\includegraphics[width=\textwidth]{images/data_mining_influential_authors.png}
    \centering(a)
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth,height=4.93cm]{images/software_engineering_influential_authors.jpeg}
    \centering{(b)}
  \end{minipage}
  \caption{\footnotesize The most influential authors (a) Data Mining (b) Software Engineering }
\end{figure}

From the information of authors, we were able to capture the organizations that were more affiliated in each domain. From the data mining domain, we can see that Google has been the top most affiliated company, then University of Minnesota, Microsoft, the University of Illinois Urbana-Champaign, the University of North California, Riverside so, and so forth. In software engineering, Microsoft has been the top most affiliated company, and then Keele University, Carnegie Mellon University, Facebook, Waterloo University so, and so forth (Figure 22). 



\begin{figure}[!tbh]
  \centering
  \begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/data_mining_frequent_affiliations.png}
    \centering(a)
    % \caption{Authorship Network}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth,height=4.93cm]{images/software_engg_frequent_affiliations.png}
    \centering(b)
    % \caption{Author Profile}
  \end{minipage}
  \caption{\footnotesize The image show the most frequently affiliated organizations involved in (a) data mining and (b) software engineering domains.}
\end{figure}

We have also explored gender and racial differences of the authors in Computer Vision and Human-Computer Interaction domain. As authors do not share any gender and race information, the only way to know is by their names. To extract the gender and racial information of authors, we have analyzed the names of the authors from census data. We have used \url{https://namecensus.com} to identify the gender and race of authors from names. We found that there are  48\% females and 52\% males in Human-Computer Interaction (Figure 23). However, we can see a major difference in Female authors involved in Computer Vision which is 40\% and 60\% male authors involved. Also, the racial difference among authors involved in these two domains is quite interesting. 

In the diagram (Figure 24), we can see that in both domains, Asian authors are around 50\% of the total numbers. The rests are 14\% Hispanic, 17\% White, and 14\% Black in Computer Vision and 49\% Asian, 19\% Hispanic, 18\% White, and 14\% Black.  

\begin{figure}[tbh]
\includegraphics[width= 9cm]{images/HCI_CV.png}
\caption{Gender Difference of Authors in (a) Human-Computer Interaction (b) Computer Vision }
\end{figure}

\begin{figure}[tbh]
\includegraphics[width= 9cm]{images/HCI_CV_1.png}
\caption{Racial Differences of Authors in (a) Human-Computer Interaction (b) Computer Vision }

\end{figure}

